Digital Twin Assisted Risk-Aware Sleep Mode Management Using Deep Q-Networks

Base stations (BSs) are the most energy-consuming segment of mobile networks. To reduce BS energy consumption, different components of BSs can sleep when BS is not active. According to the activation/deactivation time of the BS components, multiple sleep modes (SMs) are defined in the literature. In this study, we model the problem of BS energy saving utilizing multiple sleep modes as a sequential MDP and propose an online traffic-aware deep reinforcement learning approach to maximize the long-term energy saving. However, there is a risk that BS is not sleeping at the right time and incurs large delays to the users. To tackle this issue, we propose to use a digital twin model to encapsulate the dynamics underlying the investigated system and estimate the risk of decision-making (RDM) in advance. We define a novel metric to quantify RDM and predict the performance degradation. The RDM calculated by DT is compared with a tolerable threshold set by the mobile operator. Based on this comparison, BS can decide to deactivate the SMs, re-train when needed to avoid taking high risks, or activate the SMs to benefit from energy savings. For deep reinforcement learning, we use long-short term memory (LSTM), to take into account the long and short-term dependencies in input traffic, and approximate the Q-function. We train the LSTM network using the experience replay method over a real traffic data set obtained from an operator BS in Stockholm. The data set contains data rate information with very coarse-grained time granularity. Thus, we propose a scheme to generate a new data set using the real network data set which 1) has finer-grained time granularity and 2) considers the bursty behavior of traffic data. Simulation results show that using proposed methods, considerable energy saving is obtained, compared to the baselines at cost of negligible number of delayed users.

==> oldproofs.tex <==
\section{Proof Proposition 10X}\label{sec:appA}
The balance equations for state transition diagram in Figure \ref{fig:IPP} are as follows: 
When BS is in sleep mode: 
\begin{IEEEeqnarray}{lCl}
    (2\lambda + \zeta)\nu_{1,m} &=& \lambda \nu_{1,m-1} + \tau \nu_{2,m}, \quad  m \in [1,N-1]\\
    \zeta\nu_{1,m}&=&\tau \nu_{2,m}+ \lambda_2\nu_{2,m}, \quad  m \in [1,N-1]\\
     (2\lambda + \zeta)\nu_{1,0} &=& \mu u_{1,1} + \tau \nu_{2,0}\\
     \tau\nu_{2,0} &=&\mu u_{2,1} + \zeta \nu_{1,0},\\ \nonumber
     (\lambda + \zeta + \mu) u_{1,m} &=& \mu u_{1,m+1} + \lambda u_{1,m-1} + \tau u_{2,m} + \lambda \nu_{1,m-1}\\  m\in [2,N-1]\\
     (\lambda + \zeta + \mu) u_{1,1} &=& \mu u_{1,2} + \tau u_{2,1} + \lambda \nu_{1,0}
     \\\nonumber
     (\lambda + \zeta + \mu) u_{1,m} &=& \mu u_{1,m+1} + \lambda u_{1,m-1} + \tau u_{2,m}\\  m\geq N\\
     (\mu + \tau)u_{2,m} &=& \mu u_{2,m+1} + \zeta u_{1,m} +\lambda_2\nu_{2,m} \quad \nonumber\\ m \in [1,N-1]\\
          (\mu + \tau)u_{2,m} &=& \mu u_{2,m+1} + \zeta u_{1,m}  \quad m \geq N
\end{IEEEeqnarray}
Let $\kappa = 2+ \frac{\zeta\lambda_2}{\lambda(\tau + \lambda_2)}$ and $\Lambda_m=(\kappa^{m} - 2(\kappa -1)\frac{\kappa^{m-2}-1}{1-\kappa^{-1}})$ we can obtain the following equations from the balance equations:
\begin{IEEEeqnarray}{lCl}
\nu_{1,m} = &&\kappa^{-m} \nu_{1,0}\\
\nu_{1,m-1} = &&\kappa  \nu_{1,m}\\
\nu_{1,m} = &&\frac{\tau +\lambda_2}{\zeta}\nu_{2,m}\\
2\lambda \nu_{1,0} =&& \mu (u_{1,1} +u_{2,1} )
\\\nonumber
\mu\bigg(u_{1,m+1}+u_{2,m+1}\bigg) =&& \lambda\bigg(u_{1,m} + \Lambda_m \nu_{1,m}\bigg)\\
 \mu (u_{1,m+1} + u_{2,m+1}) = \lambda u_{1,m} && \quad m\geq N
\end{IEEEeqnarray}
Define $u_{1} = \sum\limits^{\infty}_{m=1} u_{1,m} + \sum\limits^{N-1}_{m=0} \nu_{1,m}= \frac{\tau}{\tau + \zeta}$ and $u_{2} = \sum\limits^{\infty}_{m=1} u_{2,m} + \sum\limits^{N-1}_{m=0} \nu_{2,m}= \frac{\zeta}{\tau + \zeta}$. By summing Equations ()-() over all possible $m$s we have: 
\begin{eqnarray}
\mu  = \lambda \bigg( u_1 + \sum^{N-1}_{m=0} (-\nu_{1,m} + \Lambda_m\nu_{2,m} )\bigg) + \mu(\sum^{N-1}_{m=0} \nu_{1,m} + \sum^{N-1}_{m=0} \nu_{2,m})
\end{eqnarray}


\begin{IEEEeqnarray}{rCl}
    \nu_{1,0} = \frac{\mu - \lambda u_{1}}{(\mu -\lambda+\frac{\mu \zeta}{\tau + \lambda_2})\sum\limits_{m=0}^{N-1} \kappa^{-m} + \lambda\sum\limits_{m=0}^{N-1}\Lambda_m\kappa^{-m}}.
\end{IEEEeqnarray}

\section{Proof Proposition 20X}\label{sec:appA1}


The probability that BS is in sleep mode is 
\begin{eqnarray}
V_s &=& \sum^{N-1}_{m=0} \bigg(\nu_{1,m} + \nu_{2,m} \bigg)\\
&=&  \Omega \nu_{1,0}
\end{eqnarray}
where $\Omega = (1+\frac{\zeta}{\tau+\lambda_2}\sum\limits_{m=0}^{N-1}\kappa^{-m})$.\\




\begin{IEEEeqnarray}{rCl}
    V_s = \frac{(\mu - \lambda u_{1})((1+\frac{\zeta}{\tau+\lambda_2}\sum\limits_{m=0}^{N-1}\kappa^{-m}))}{(\mu -\lambda+\frac{\mu \zeta}{\tau + \lambda_2})\sum\limits_{m=0}^{N-1} \kappa^{-m} + \lambda\sum\limits_{m=0}^{N-1}\Lambda_m\kappa^{-m}} \\\nonumber\qed
\end{IEEEeqnarray}

\section{Proof Proposition 2}\label{sec:appB}
The average number of users in the BS, when it is in sleep mode is calculated by,
\begin{IEEEeqnarray}{rCl}
U_s &=& \sum\limits_{m=0}^{N-1} m \nu_{1,m} + \sum\limits_{m=0}^{N-1} m \nu_{2,m}\\
&=& \bigg( \frac{\tau + \lambda_2 + \zeta}{\tau+ \lambda_2}  \sum\limits_{m=0}^{N-1} m\kappa^{-m} \bigg) \nu_{1,0}\\\nonumber
&=& \bigg(\frac{\tau + \lambda_2 + \zeta}{\tau+ \lambda_2}\bigg)\bigg(\frac{\kappa(1-\kappa^{-(N-1)})-N(\kappa -1)\kappa^{-(N-1)}}{(\kappa -1)^2}\bigg)\nu_{1,0}\\
\end{IEEEeqnarray}

Based on little's formula, average delay of users when BS is in the sleep mode  is 
\begin{IEEEeqnarray}{rCl}
\overline{d}& = & \frac{U_s}{ \frac{\tau}{\tau+\zeta}\lambda}
\end{IEEEeqnarray}


\section{Proof Proposition 4}\label{sec:appC}
The probability that BS is in the sleep mode and no user is in the system is

\begin{IEEEeqnarray}{rCl}
V_s(\textit{sleep}| \textit{no user}) &=& \nu_{1,0} + \nu_{2,0} \\
&=& \frac{\tau + \zeta + \lambda_2}{\tau + \lambda_2}\nu_{1,0}
\end{IEEEeqnarray}
The duration of staying in this case is 

\begin{IEEEeqnarray}{rCl}
T_s(\textit{sleep}| \textit{no user}) &=& \nu_{1,0} + \nu_{2,0} \\
&=& \frac{\tau + \lambda_2}{(\tau + \zeta + \lambda_2)\nu_{1,0}}
\end{IEEEeqnarray}

%%%

\section{Proof Proposition 5}\label{sec:appE}
The number of times that BS activate or deactivate its components is derived as, 

\begin{IEEEeqnarray}{rCl}
F_m &=& 2(\lambda\sum\limits_{m=0}^{N-1}\nu_{1,m} +\lambda_2\sum\limits_{m=0}^{N-1}\nu_{2,m} )\\
&=& 2 \nu_{1,0} (\lambda + \frac{\zeta}{\tau+ \lambda_2}\lambda_2)\sum\limits_{m=0}^{N-1}\kappa^{-m}
\end{IEEEeqnarray}


